StoreBench: A Live-Commerce Environment for Evaluating and Training Autonomous Operator Agents

Reinforcement learning environments are now a primary lever for improving large language model (LLM) capabilities in post-training, yet most agentic benchmarks remain static: the world moves only when the agent acts, the reward is a terminal verdict, and the pass bar is set arbitrarily. We introduce StoreBench, a live-commerce environment in which an agent runs a mid-size online apparel store on a production-grade commerce backend, testing long-horizon planning and economic judgment under uncertainty. Customers order around the clock, suppliers reprice and fail, and market shocks arrive with partial or no warning. The agent acts through the same 29 merchant tools a human operator would use, under a windowed operation budget that makes simulated time a function of actions taken, so model latency cannot influence simulated time. Pass thresholds are calibrated against scripted anchor policies, the reward is hardened against a catalogue of reward hacks, and every episode replays identically given a sequence of actions. We evaluate seven frontier LLMs on 11 scenarios of 30 to 45 days and a full simulated year, over three world seeds at matched reasoning effort. No model matches the scripted smart-triage policy on average: the best, DeepSeek-V4-Pro, passes 49% of task-seed cells against the heuristic's 97%. Human experts working through the same tools and budgets outscore every model (mean composite 0.708 vs. 0.700). Over a full simulated year under the Claude Code harness, most models show dramatic performance improvement. In a GRPO post-training run, Qwen3.5-27B trained on only five disjoint tasks raises its mean composite on the held-out evaluation tasks from 0.136 to 0.373. We release five example training-split tasks, ten sample trajectories, and the scoring and verification tooling; the full environment and evaluation suite are withheld to keep the benchmark uncontaminated.

==> figures/ladder_schematic.tex <==
% Figure: the anchor ladder as an annotated score axis. Positions use
% suite-mean composites; x = 14 * composite.
\begin{tikzpicture}[
  font=\small,
  anchorlbl/.style={font=\scriptsize, align=center},
  gatelbl/.style={font=\scriptsize\itshape, align=center},
  stem/.style={thick},
  gate/.style={{Stealth[length=1.6mm]}-{Stealth[length=1.6mm]}, thin},
]
% score axis
\draw[-{Stealth[length=2.5mm]}, thick] (-0.5, 0) -- (12.3, 0)
  node[anchorlbl, right=1mm] {composite};

% honest anchors: stem + dot + label (staggered heights near zero)
\foreach \x/\h/\name/\val in {
  0/0.55/do-nothing/0.00,
  1.4/1.15/absentee/0.10,
  6.48/0.55/blast-list/0.46,
  8.93/0.55/rule-based/0.64,
  10.70/1.15/smart-triage/0.76}{
  \draw[stem] (\x, 0) -- (\x, \h);
  \fill (\x, 0) circle (1.6pt);
  \node[anchorlbl, above] at (\x, \h) {\name\\(\val)};
}

% exploiter: forced below every honest anchor
\draw[stem, red!70!black] (0.55, 0) -- (0.55, 1.75);
\fill[red!70!black] (0.55, 0) circle (1.6pt);
\node[anchorlbl, above, text=red!70!black] at (0.55, 1.75)
  {exploiter\\(0.04)};
\node[gatelbl, anchor=west, text=red!70!black] at (-0.4, 2.5)
  {gate (iv): exploiter below every honest anchor};

% pass threshold
\draw[red!70!black, dashed, very thick] (9.81, -0.55) -- (9.81, 1.85);
\node[anchorlbl, above, text=red!70!black, fill=white, inner sep=1pt]
  at (9.81, 1.9) {\textbf{pass threshold (0.70)}\\midpoint of the two
  best\\honest anchors};

% gates below the axis
\draw[gate] (6.48, -0.45) -- (8.93, -0.45);
\node[gatelbl, below] at (7.70, -0.5) {judgment gap (gate ii)};
\draw[gate] (8.93, -0.45) -- (9.75, -0.45);
\draw[gate] (9.87, -0.45) -- (10.70, -0.45);
\node[gatelbl, below] at (10.6, -0.5) {flap margins (gate iii)};

% zero and scale
\draw[-{Stealth[length=1.6mm]}, thin] (1.4, -1.15) -- (1.4, -0.1);
\node[gatelbl, below] at (1.4, -1.15) {$z$ (zero)};
\draw[decorate, decoration={brace, mirror, amplitude=4pt}]
  (1.4, -1.75) -- (10.70, -1.75);
\node[gatelbl, below] at (6.05, -1.95)
  {$s$ (scale): absentee to best anchor};
\end{tikzpicture}


==> figures/metering.tex <==
% Figure: windowed operation metering. One window's budget spends down;
% exhausting it (or end_window) advances the world one step.
\begin{tikzpicture}[
  font=\small,
  op/.style={draw, minimum height=6.5mm, minimum width=13mm, inner sep=2pt,
             align=center, font=\scriptsize},
  free/.style={op, fill=black!5, dashed},
  world/.style={draw, rounded corners=2pt, align=center, inner sep=4pt,
                fill=black!8, minimum height=15mm},
  arr/.style={-{Stealth[length=2mm]}, thick},
  lbl/.style={font=\scriptsize, align=center},
]
% window bracket
\node[lbl, anchor=west] at (0, 1.35) {\textbf{Window $k$}
  (12 simulated hours; clock frozen while the agent deliberates)};

% op slots
\node[free] (s) at (0.8, 0) {\texttt{status}\\(free)};
\node[op, right=1.5mm of s] (o1) {read\\report};
\node[op, right=1.5mm of o1] (o2) {set\\price};
\node[op, right=1.5mm of o2] (o3) {place\\PO};
\node[op, right=1.5mm of o3] (o4) {ship\\order};
\node[op, right=1.5mm of o4] (o5) {refund\\return};
\node[lbl, right=2mm of o5] (dots) {$\cdots$};
\node[op, right=2mm of dots] (oN) {op\\$B_k/B_k$};

% budget annotation
\draw[decorate, decoration={brace, mirror, amplitude=3pt}]
  ([yshift=-1.5mm]o1.south west) -- ([yshift=-1.5mm]oN.south east)
  node[lbl, midway, below=2mm] {each call spends 1 operation from the window
  budget $B_k$ (11 to 20); budgets do not roll over};

% world advance
\node[world, right=25mm of oN] (world) {\textbf{World advances}\\
  \scriptsize demand lands $\cdot$ deliveries progress\\
  \scriptsize returns escalate $\cdot$ events fire};
\draw[arr] (oN) -- node[lbl, above, pos=0.5, yshift=1.5mm] {budget spent\\
  or \texttt{end\_window}} (world);

% loop back to next window: over the window label, down the left edge
\draw[arr, rounded corners=3pt] (world.north)
  |- node[lbl, above, pos=0.7] {window $k{+}1$: fresh budget, new
  obligations} (-1.1, 1.8) -- (-1.1, 0) -- (s.west);
\end{tikzpicture}


==> sections/gen_fullyear.tex <==
% AUTO-GENERATED by results_gen.py -- do not edit by hand.
% Regenerated 2026-09: canonical full-year (claude-code harness, extended thinking,
% n=9 = 3 seeds x 3), matched-effort short-horizon mean in the Short column.
% Data source for make_horizon_figure.py; the last column is the long-horizon outcome
% (clean / premature exit / idle-delegation), not an operating-mode label.
\begin{table}[t]
\centering
\caption{Long horizon vs. short horizon. On the 365-window \emph{full-year} task, run under an agentic harness with extended thinking and compaction, the capable short-horizon models sustain near-oracle operation over the whole year, while two models show genuine long-horizon failures. $\Delta$ is full-year minus the (matched-effort, goose) short-horizon mean; the two regimes differ in harness and effort, so $\Delta$ contrasts them rather than isolating horizon.}
\label{tab:fullyear}
\begin{tabular}{lrrrl}
\toprule
Model & Short & Full-year & $\Delta$ & Outcome \\
\midrule
DeepSeek-V4-Pro & 0.700 & 0.976 & +0.276 & clean \\
Qwen3.8-Max & 0.587 & 0.974 & +0.387 & clean \\
Claude Opus 4.8 & 0.668 & 0.971 & +0.303 & clean \\
Claude Fable 5 & 0.629 & 0.966 & +0.337 & clean \\
Muse Spark 1.2 & 0.387 & 0.862 & +0.475 & clean \\
GPT-5.6 Sol & 0.538 & 0.783 & +0.245 & early \\
Gemini 3.8 Flash & 0.552 & 0.496 & -0.056 & idle \\
\bottomrule
\end{tabular}
\end{table}

